Performance Metric Elicitation from Pairwise Classifier Comparisons

Given a binary prediction problem, which performance metric should the classifier optimize? We address this question by formalizing the problem of Metric Elicitation. The goal of metric elicitation is to discover the performance metric of a practitioner, which reflects her innate rewards (costs) for correct (incorrect) classification. In particular, we focus on eliciting binary classification performance metrics from pairwise feedback, where a practitioner is queried to provide relative preference between two classifiers. By exploiting key geometric properties of the space of confusion matrices, we obtain provably query efficient algorithms for eliciting linear and linear-fractional performance metrics. We further show that our method is robust to feedback and finite sample noise.

==> algorithms.tex <==
\section{Algorithms}
\label{sec:algorithms}

In this paper, we primarily deal with the three types of metrics - linear, concave, and linear fractional. We assume that all the metrics are bounded over the set $\Ccal$, and monotonically increasing in TP and TN. All the metric examples discussed in the section \ref{sec:background} have this property. It is reasonable to assume the monotonic increasing property in TP and TN; however, in the supplement section we also discuss how to elicit the performance metric when it is monotonic but decreasing in TP and TN, for the linear and the concave case.  

\subsection{Eliciting Linear Performance Metric}
\label{ssec:elicit_linear}

As discussed before, suppose that the oracle performance metric is of the linear form, which is unknown to the learning/eliciting agent: 

\bequation
\phi^*(tp, tn) = \langle \mmbf^*, (tp, tn) \rangle + m_0^*
\eequation

Since the metric needs to be bounded, without loss of generality, we take $\norm{\mmbf^*} =1$ and $m_0^* = 0$ as it does not matter from the elicitation point of view. Further, we take the case of monotonic increasing, which implies $m_{11}, m_{00} \geq 0$. The optimal confusion matrix is $C^* = (TP^*, TN^*)$. We denote the quantity $\langle \mmbf^*, (TP^*, TN^*) \rangle$ as $C_0$. We observe the following: given two confusion matrices $C$ and $C'$, whenever the oracle is asked a query of the type $\Omega(C, C')$, following is the equivalence:

\begin{align}
		\Omega(C, C') &= \1[\phi^*(C) > \phi^*(C')] \nonumber \\
 			  &= \1[\langle \mmbf^*, (TP, TN)_C \rangle > \langle \mmbf^*, (TP, TN)_{C'} \rangle] \nonumber  \\
 			  &= \1[\langle \mmbf^*, (TP, TN)_C \rangle + C_0 > \langle \mmbf^*, (TP, TN)_{C'} \rangle] + C_0] \nonumber \\
 			  &= \1[\frac{\langle \mmbf^*, (TP, TN)_C \rangle + C_0}{\norm{\mmbf^*}} > \frac{\langle \mmbf^*, (TP, TN)_{C'} \rangle] + C_0}{\norm{\mmbf^*}}] \\nonumber
\end{align}

Assuming the positive orthant direction to be positive for the normal vector, the quantity  $\langle \mmbf^*, (TP, TN) \rangle \leq 0 \forall \; (TP, TN) \in \Ccal$. This is because $\langle \mmbf^*, (TP^*, TN^*) \rangle  = C_0$ is the equation of a supporting hyperplane with slope $-\frac{m_{11}}{m_{00}}$ (See \eqref{eq:support}). This implies:

\begin{align}
	\Omega(C, C') &=  \1[\frac{\langle \mmbf^*, (TP, TN)_C \rangle + C_0}{\norm{\mmbf^*}} > \frac{\langle \mmbf^*, (TP, TN)_{C'} \rangle] + C_0}{\norm{\mmbf^*}}] \nonumber \\
				&= -|\frac{\langle \mmbf^*, (TP, TN)_C \rangle + C_0}{\norm{\mmbf^*}}| > -|\frac{\langle \mmbf^*, (TP, TN)_{C'} \rangle] + C_0}{\norm{\mmbf^*}}| \nonumber \\
				&= \1[d(C) < d(C')]
	\label{eq:distance}
\end{align}

where, $d : \Ccal \times \Lcal \rightarrow \R{} $ is the distance of a confusion matrix $C$ from a hyperplane $\ell$. 

\bprop
Fix a hyperplane $\ell := m_{11}tp + m_{00}tn = C_0$. Again, $m_{11}, m_{00} \geq 0$ and $\norm{\mmbf} = 1$. The restriction of $d$ over the set of $(\partial \Ccal)_+$ is unimodal (only one local minimum). Similar case holds true for the lower  boundary provided $m_{11}, m_{00} < 0$ and $\norm{\mmbf} = 1$.
\eprop

This observation allows us to create an efficient binary search algorithm \ref{alg:linear} to elicit the performance metric in the linear case. We show the behavior of function $d$ given a true metric $\phi^*$ defined by $\theta^*$ over the $\theta \in [0, 2\pi]$ in Figure \ref{fig:distance} \textbf{Add Figure}. 

\balgorithm[t]
	\caption{Binary Search for LPM Elicitation}
	\label{alg:linear}
	\balgorithmic[1]
		\STATE \textbf{Input:} $\epsilon > 0$.
		\STATE \textbf{Initialize:} $\theta_a = 0$, $\theta_b = \frac{\pi}{2}$
		\WHILE {$\theta_b - \theta_a > \epsilon$}
		\STATE Set $\gamma = \frac{\theta_a + \theta_b}{2}$.
		\STATE Obtain the hyperplane $\ell_{\gamma - \epsilon}$, $\ell_{\gamma}$, and $\ell_{\gamma + \epsilon}$.
		\STATE Obtain the Bayes optimal classifier $h^*_{\gamma - \epsilon})$, $h^*_{\gamma}$, and $h^*_{\gamma + \epsilon}$ using Proposition \ref{pr:bayeslinear}.
		\STATE Obtain the corresponding Bayes optimal confusion matrix $C^*_{\gamma - \epsilon}$, $C^*_{\gamma}$, and $C^*_{\gamma + \epsilon}$.
		\STATE Ask queries $\omega_1 = \Omega(C^*_{\gamma - \epsilon}, C^*_{\gamma})$ and $\omega_2 = \Omega(C^*_{\gamma}, C^*_{\gamma + \epsilon})$.
		\IF{$\omega_1 = 0$ and $\omega_2 = 0$}
			\STATE Set $\theta_a = \theta_\gamma$
		\ELSIF{$\omega_1 = 1$ and $\omega_2 = 1$}
			\STATE Set $\theta_b = \theta_\gamma$.
		\ELSE
			\STATE Set $\theta_a = \frac{\theta_\gamma + \theta_a}{2}$.
			\STATE Set $\theta_b = \frac{\theta_\gamma + \theta_b}{2}$.
		\ENDIF
		\ENDWHILE
		\STATE\textbf{Output:} $\theta_\gamma$.
	\ealgorithmic
\ealgorithm

Since for any unit normal defined as $(\cos\theta, \sin\theta)$, we can find a supporting hyperplane of the convex set passing through one unique point $\partial C_+$. This boundary point essentially maximizes the linear objective function, where $m_{11} = \cos\theta$ and $m_{00} = \sin\theta$. Algorithm \ref{alg:linear} essentially searches over the normal, for which the corresponding supporting hyperplane's optimal point's distance (as defined in \eqref{eq:distance}) is close to 0. 

We start with the interval $[\theta_a = 0, \theta_b = \frac{\pi}{2}]$. We define three $\theta$ values near the mid point $\theta_\gamma$ of the interval: $\theta_\gamma - \epsilon$, and $\theta_\gamma + \epsilon$. In line 5, we figure out the hyperplanes corresponding to these three $\theta$ values. Given the hyperplanes (or the set of $m_{11}$ and $m_{00}$), we compute the optimal classifiers for these hyperplanes in line 6 using Proposition \ref{pr:bayeslinear}. In line 7, we compute the Bayes optimal confusion matrices corresponding to the optimal classifiers. Then, we pose two queries to the oracle in line 8. In lines 9-15, we shrink the search interval by half depending on the answers by the oracle.

Notice that even if the oracle's metric is monotonically decreasing in TP and TN, we can still figure out the true metric by posing 4 additional queries to fix the quadrant of search. We can ask $\Omega(C^*_0, C^*_{\frac{\pi}{4}})$, $\Omega(C^*_{\frac{\pi}{4}}, C^*_{\frac{\pi}{2}})$, $\Omega(C^*_\pi, C^*_{\frac{5\pi}{4}})$, and $\Omega(C^*_{\frac{5\pi}{4}}, C^*_{2\pi})$. This will allow us to know the quadrant where the function $d$ is decreasing and then increasing. After knowing this, we only to need to figure out the point where $d(C^*) < \epsilon$, which can be done using the above algorithm.

\btheorem
Given $\epsilon > 0$, Algorithm \ref{alg:linear} obtains a $\hat{\theta}$ (or say, $\hat{\ell}$) which is $\epsilon$ radians away from the true $\theta^*$ in $2\log(\frac{1}{\epsilon})$ queries to the oracle, when the true metric is monotonically increasing (or decreasing). In general, Algorithm \ref{alg:linear} requires $2\log(\frac{1}{\epsilon}) + 4$ queries to achieve the same.  
\etheorem
